Abstraction-Free Control Synthesis to Satisfy Temporal Logic Constraints under Sensor Faults and Attacks

We study the problem of synthesizing a controller to satisfy a complex task in the presence of sensor faults and attacks. We model the task using Gaussian distribution temporal logic (GDTL), and propose a solution approach that does not rely on computing any finite abstraction to model the system. We decompose the GDTL specification into a sequence of reach-avoid sub-tasks. We develop a class of fault-tolerant finite time convergence control barrier functions (CBFs) to guarantee that a dynamical system reaches a set within finite time almost surely in the presence of malicious attacks. We use the fault-tolerant finite time convergence CBFs to guarantee the satisfaction of `reach' property. We ensure `avoid' part in each sub-task using fault-tolerant zeroing CBFs. These fault-tolerant CBFs formulate a set of linear constraints on the control input for each sub-task. We prove that if the error incurred by system state estimation is bounded by a certain threshold, then our synthesized controller fulfills each reach-avoid sub-task almost surely for any possible sensor fault and attack, and thus the GDTL specification is satisfied with probability one. We demonstrate our proposed approach using a numerical study on the coordination of two wheeled mobile robots.

==> formulation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem Formulation}\label{sec:formulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Consider a continuous-time control-affine system
\begin{equation}\label{eq:dynamic}
    \dot{x}=f(x)+g(x)(u+a),\quad x(0)=x_0,
\end{equation}
where $x\in\mathcal{X}\subseteq\mathbb{R}^n$ is the system state, and $u\in\mathcal{U}\subseteq\mathbb{R}^m$ is the control input provided by the controller, and $a\in\mathcal{A}\subseteq\mathbb{R}^m$ the signal injected by a malicious adversary. The initial state at time $t=0$ is denoted as $x(0)=x_0$. Vector fields $f$ and $g$ are locally Lipschitz continuous. 

We assume that the controller can fully observe the system state $x$. At each time $t\geq 0$, it commits to a randomized control policy $\mu:\mathcal{X}\rightarrow\Delta(\mathcal{U})$, mapping from the state space to the set of control inputs, where $\Delta(\mathcal{U})$ denotes the set of probability distributions over $\mathcal{U}$.

We consider the scenarios where there exists a malicious adversary that injects signal $a$ into the actuator of system \eqref{eq:dynamic}. We assume that the interaction pattern between the controller and adversary follows the Stackelberg setting where the controller is the leader and the adversary is the follower, i.e., the adversary knows the policy committed by the controller. We denote the information available to the adversary as $\mathcal{I}_A=\{\mu\}\cup\{x\}$. The attack signal $a$ is then computed by the adversary following attack policy $\tau:\mathcal{I}_A\rightarrow \mathcal{A}$.

Let $\Pi$ be a finite set of atomic propositions. We define a labeling function $L:\mathcal{X}\mapsto 2^\Pi$ that maps any state $x\in\mathcal{X}$ to a subset of atomic propositions that hold true at $x$. We also define $\llbracket\pi\rrbracket=\{x|\pi\in L(x)\}$ to be the set of states that satisfies the atomic proposition $\pi\in\Pi$. In this work, we assume that $\llbracket\pi\rrbracket$ is a closed set for all $\pi\in\Pi$, and $\llbracket\pi\rrbracket$ can be represented as $\llbracket\pi\rrbracket=\{x|Z_\pi(x)\geq 0\}$, where $Z_\pi:\mathbb{R}^n\mapsto\mathbb{R}$ is a bounded and continuously differentiable function. 
We slightly overload the notation $\llbracket\cdot\rrbracket$, and define the states that satisfy a subset of atomic propositions $P\in 2^\Pi$ as 
\begin{equation}\label{eq:subset atomic}
    \llbracket P\rrbracket=\begin{cases}
    \mathcal{X}\setminus\cup_{\pi\in\Pi}\llbracket\pi\rrbracket&\mbox{ if }P=\emptyset\\
    \cap_{\pi\in P}\llbracket\pi\rrbracket\setminus\cup_{\pi\in\Pi\setminus P}\llbracket\pi\rrbracket&\mbox{ otherwise}
    \end{cases}
\end{equation}
That is, $\llbracket P\rrbracket$ is the subset of system states $\mathcal{X}$ that satisfy all and only propositions in $P$ \cite{wongpiromsarn2015automata}.
% Similarly, we denote the set of states on the boundary of $\llbracket\pi\rrbracket$ and inside $\llbracket\pi\rrbracket$ as
% \begin{equation*}
%     B(\llbracket\pi\rrbracket)=\{x|h_\pi(x)= 0\},\quad Int(\llbracket\pi\rrbracket)=\{x|h_\pi(x)> 0\},
% \end{equation*}
% where $B(\cdot)$ and $Int(\cdot)$ denote the boundary and interior of a set, respectively.

We define the trajectory of system \eqref{eq:dynamic} as $\mathbf{x}:[0,\infty)\mapsto\mathcal{X}$ that maps from any time $t\geq0$ to the system state $x(t)$. 
We then define the trace of a trajectory $\mathbf{x}$ as follows.
\begin{definition}[Trace of Trajectory \cite{wongpiromsarn2015automata}]\label{def:trace}
An infinite sequence $Trace(\mathbf{x})=P_0,P_1,\ldots$, where $P_i\in 2^\Pi$ for all $i=0,1,\ldots$ is a trace of a trajectory $\mathbf{x}$ if there exists an associated time sequence $t_0,t_1,\ldots$ of time instants such that
\begin{enumerate}
    \item $t_0=0$
    \item $t_\tau\rightarrow\infty$ as $\tau\rightarrow\infty$
    \item $t_i<t_{i+1}$
    \item $x(t_i)\in \llbracket P_i\rrbracket$
    \item if $P_i\neq P_{i+1}$, then there exists some $t_i'\in[t_i,t_{i+1}]$ such that $x(t)\in\llbracket P_i\rrbracket$ for all $t\in(t_i,t_i')$, $x(t)\in\llbracket P_{i+1}\rrbracket$ for all $t\in(t_i',t_{i+1})$, and either $x(t_i')\in\llbracket P_i\rrbracket$ or $x(t_i')\in\llbracket P_{i+1}\rrbracket$.
\end{enumerate}
\end{definition}
The trace of the system trajectory gives the sequence of atomic propositions satisfied by the system, and thus bridges the system behavior with temporal logic specification. Given a controller $\mu$, we denote the trajectory under controller $\mu$ and attack policy $\tau$ as $\mathbf{x}^{\mu\tau}$. The trace of trajectory $\mathbf{x}^{\mu\tau}$ is denoted by $Trace(\mathbf{x}^{\mu\tau})$. Suppose a specification $\varphi$ belonging to $\text{LTL}_{\setminus\bigcirc}$ is given to system \eqref{eq:dynamic}. If $Trace(\mathbf{x}^{\mu\tau})\models\varphi$, we say system \eqref{eq:dynamic} satisfies $\varphi$ under controller $\mu$, or controller $\mu$ satisfies $\varphi$. 
% We say policy $\mu$ is an \emph{almost sure} policy if the probability of satisfying $\varphi$ is one using policy $\mu$.
We state the problems of interest as follows.
\begin{problem}\label{prob:formulation 2}
Compute a randomized policy for the controller $\mu:\mathcal{X}\rightarrow\mathcal{U}$ under which system \eqref{eq:dynamic} satisfies the given LTL specification $\varphi$ belonging to $LTL_{\setminus\bigcirc}$ with probability no less than $1-\epsilon$, given that the adversary plays its best response to $\mu$.
\end{problem}


==> formulation_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem Formulation}\label{sec:formulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Consider a nonlinear dynamical system defined as
\begin{subequations}\label{eq:dynamics}
\begin{align}
    dx_t &= (f(x_t)+g(x_t)u_t)dt+\sigma_tdW_t,\\
    dy_t &= (cx_t+a_t)dt+\nu_tdV_t
\end{align}
\end{subequations}
where $x_t\in\mathbb{R}^n$ is the system state, and $u_t\in\mathbb{R}^p$ is the control input at time t. Functions $f:\mathbb{R}^n\rightarrow\mathbb{R}^n$ and $g:\mathbb{R}^n\rightarrow\mathbb{R}^{n\times p}$ are locally Lipschitz continuous, $\sigma_t\in\mathbb{R}^{n\times n}$, $W_t$ is an $n$-dimensional Brownian motion, $y_t\in\mathbb{R}^q$ is the output at time $t$, $c\in\mathbb{R}^{q\times n}$, $a_t\in\mathbb{R}^q$ is the attack signal injected by an adversary, $\nu_t\in\mathbb{R}^{q\times q}$, and $V_t$ is a $q$-dimensional Brownian motion.

We assume that the system operates in the presence of a malicious adversary. The adversary can inject a signal $a_t$ to manipulate the output with $supp(a_t)\subseteq\{1,\ldots,q\}$. We assume that once the adversary determines the set of sensors to attack, it cannot adjust the support of the attack signal, i.e., the adversary cannot change its target once the attack started. We also assume that there are finitely many choices for the support of $a_t$, denoted as $\mathcal{F}$, which is also known to the system. However, the choice $supp(a_t)$ made by the adversary is not known to the system.

The system employs an EKF to estimate the system state (see Section \ref{sec:EKF}). We denote the state estimate at time $t$ as $\hat{x}_t$ and denote the estimate error covariance as $P_t$. A belief state $b_t$ is defined as $b_t=(\hat{x}_t,P_t)$.

The system is given a GDTL specification that needs to be satisfied. We define a labeling function $L:\mathbb{R}^n\times \mathbb{R}^{n\times n}\rightarrow 2^\Pi$, where $\Pi$ is a set of atomic propositions. Note that the system does not know the system state $x_t$ directly. Instead, the system maintains an estimate $\hat{x}_t$ over the system state, and thus the satisfaction of each atomic proposition should be evaluated using the state estimate. Let $Z\in 2^\Pi\cup \mathcal{L}_\varphi$. We define $\llbracket Z\rrbracket=\{b=(\hat{x},P):\pi\in L(\hat{x}) \lor l(b)\leq 0\land \pi'\notin L(\hat{x}) \land l'(b)> 0 \text{ with }\pi,l\in Z, \pi',l'\notin Z\}$.

We let $\mathbf{b}$ be a trajectory of belief state of infinite length and $\mathbf{b}^t$ be the suffix of $\mathbf{b}$ starting from time $t$.
\begin{definition}[Trace of Trajectory \cite{wongpiromsarn2015automata}]\label{def:trace}
An infinite sequence $Trace(\mathbf{b})=Z_0,Z_1,\ldots,Z_i,\ldots$, where $Z_i\in 2^\Pi$ for all $i=0,1,\ldots$ is a trace of a trajectory $\mathbf{b}$ if there exists an associated sequence $t_0,t_1,\ldots,t_i,\ldots$ of time instants such that
\begin{enumerate}
    \item $t_0=0$
    \item $t_i\rightarrow\infty$ as $i\rightarrow\infty$
    \item $t_i<t_{i+1}$
    \item $\hat{x}_{t_i}\in \llbracket Z_i\rrbracket$
    \item if $Z_i\neq Z_{i+1}$, then there exists some $t_i'\in[t_i,t_{i+1}]$ such that $\hat{x}_t\in\llbracket Z_i\rrbracket$ for all $t\in(t_i,t_i')$, $\hat{x}_t\in\llbracket Z_{i+1}\rrbracket$ for all $t\in(t_i',t_{i+1})$, and either $\hat{x}_{t_i'}\in\llbracket Z_i\rrbracket$ or $\hat{x}_{t_i'}\in\llbracket Z_{i+1}\rrbracket$.
\end{enumerate}
\end{definition}
Using the trace of system trajectory, we have that GDTL specification $\varphi$ is satisfied if $Trace(\mathbf{b})\models \varphi$. The problem investigated in this paper is then formulated as follows.
\begin{problem}\label{prob:formulation}
Given a parameter $\epsilon\in(0,1)$, compute a control policy $\mu:\{y_{t'}:t'\in[0,t)\}\rightarrow\mathbb{R}^p$ for the system at each time $t$ mapping from the sequence of outputs to a control input $u_t$, so that the probability of satisfying $\varphi$, denoted as $\mathbb{P}(\varphi)$, is lower bounded by $1-\epsilon$.
\end{problem}

==> intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Cyber-physical systems (CPS) have found their applications in multiples domains where increasingly complex tasks need to be achieved. Typical examples include autonomous vehicles, industrial control systems, and robotics. Temporal logics \cite{baier2008principles} such as linear temporal logic have emerged to assign tasks to CPS because of their concreteness, rigor, and rich expressiveness. To model the process noise and observation noise that are normally incurred by CPS in practice, Gaussian distribution temporal logic (GDTL) has been proposed to specify CPS properties involving the uncertainties in the system state \cite{vasile2016control,leahy2019control}. Controller design for CPS under different temporal logic constraints has attracted extensive research attention \cite{kress2009temporal,coogan2015traffic,vasile2016control,leahy2019control}. There have been two trends of research for temporal logic based control synthesis, namely the \emph{abstraction-based approaches} and \emph{abstraction-free approaches}. 

The abstraction-based approaches \cite{fainekos2009temporal,ding2014optimal,wongpiromsarn2009receding,vasile2016control,leahy2019control,kress2009temporal,coogan2015traffic} are motivated by formal methods in the context of model checking \cite{baier2008principles}. These approaches translate the system model from continuous domain to discrete domain by computing a finite abstraction. Typical examples of finite abstractions include finite transition systems \cite{fainekos2009temporal} and Markov decision processes (MDPs) \cite{ding2014optimal,wongpiromsarn2009receding}. These abstractions can be generated by partitioning the state and control input spaces with property preserving guarantees such as bisimulation \cite{alur2000discrete}. Using the abstractions,  control synthesis for temporal logic specifications is achieved by first taking the Cartesian product between the abstractions and the automaton that represents the temporal logic specification, and then applying the modeling checking algorithms. In general, the abstraction-based approaches are computationally demanding and suffer from the curse of dimensionality.

To mitigate the computation required by the abstraction-based approaches, abstraction-free approaches are proposed. Abstraction-free synthesis eliminates the step on constructing the finite abstractions, and directly computes the controller in the continuous domain \cite{wolff2012robust,horowitz2014compositional,papusha2016automata,srinivasan2018control,lindemann2018control,yang2019continuous,niu2020control}. These approaches decompose the given temporal logic specification into a sequence of problems of smaller scales, and utilize more computationally efficient techniques to solve each of them \cite{srinivasan2018control,lindemann2018control,yang2019continuous,niu2020control}. In particular, control barrier function (CBF)-based approaches \cite{ames2014control}, which convert the control synthesis at each time step to a linear constraint in the control input, have gained increasing research attention due to their ease of implementation.


The previously introduced abstraction-based approaches \cite{fainekos2009temporal,ding2014optimal,wongpiromsarn2009receding,vasile2016control,leahy2019control,kress2009temporal,coogan2015traffic} and abstraction-free approaches \cite{wolff2012robust,horowitz2014compositional,papusha2016automata,srinivasan2018control,lindemann2018control,yang2019continuous,niu2020control} assume that there exist no faults or malicious attack targeting at CPS. However, CPS have been shown to be vulnerable to sensor faults and malicious attacks \cite{liu2011false,mo2010false,cardenas2008research,fawzi2014secure}, making temporal logic based control synthesis even more challenging due to the following reasons. First, sensor faults and malicious attacks can arbitrarily manipulate the sensor measurements. Inaccurate measurements prevent the CPS from correctly evaluating and tracking the satisfaction of temporal logic specifications. Moreover, the faulty or compromised measurements can bias the state estimate and lead to erroneous controller output, which deviates the system trajectory and cause violation of the temporal logic specification. Although there has been research attention fault and attack detection \cite{mo2010false,shoukry2017secure,fawzi2014secure} and low-level control design under sensor attacks \cite{clark2018linear}, abstraction-free temporal logic based control synthesis in the presence of sensor faults and attacks, however, has not been studied yet.

In this paper, we study the problem of synthesizing a controller for a nonlinear control-affine system to satisfy a GDTL specification. The system is subject to process and observation noises. Moreover, there exists a malicious adversary that can arbitrarily manipulate the sensor measurements of the system. We decompose the GDTL specification into a sequence of reach-avoid problems with the system state uncertainties being explicitly encoded. We then derive a sufficient condition for the system controller to satisfy each decomposed problem. We develop a class of fault-tolerant finite time convergence CBFs, combined with the recently proposed fault-tolerant zeroing CBF \cite{clark2020control}, to guarantee the satisfaction of each decomposed reach-avoid requirement. We make the following specific contributions:
\begin{itemize}
    \item We develop fault-tolerant finite time convergence CBFs which guarantee the finite time convergence in probability in the presence of sensor faults and attacks.
    \item We derive a set of sufficient conditions for the controller using fault-tolerant finite time convergence CBFs and fault-tolerant zeroing CBFs so as to solve each decomposed reach-avoid problem. 
    \item We prove that the derived controller guarantees that each decomposed reach-avoid problem can be satisfied with probability one, provided the accuracy bounds of the extended Kalman filters used by the system. We further show the almost sure satisfaction guarantee on the GDTL specification using our proopsed approach.
    \item We evaluate our proposed approach using a numerical case study on a wheeled robot.
\end{itemize}

The rest of this paper is organized as follows. The related work is presented in Section \ref{sec:related}. Section \ref{sec:prelim} presents the system model and reviews necessary background on extended Kalman filter and GDTL. Section \ref{sec:sol} presents our proposed solution approach. A numerical case study is presented in Section \ref{sec:simulation}. We conclude the paper in Section \ref{sec:conclusion}. Background on finite time stability in probability is reviewed in Appendix.







==> prelim.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}\label{sec:preliminary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This section presents background on Gaussian distribution temporal logic (GDTL) and finite time stability of stochastic nonlinear systems.

\subsection{Notations}
Throughout this paper, we use $\mathbb{R}^n$ to denote the $n$-dimensional Euclidean space. Given a vector $a\in\mathbb{R}^n$, we use $supp(a)$ to denote its support. For any matrix $A$, we denote its trace as $tr(A)$. We denote the set of non-negative real numbers as $\mathbb{R}_{\geq 0}$. For a set $\mathcal{C}\subseteq\mathbb{R}^n$, we denote its interior as $Int(\mathcal{C})$. A function $\alpha:\mathbb{R}_{\geq 0}\rightarrow\mathbb{R}_{\geq 0}$ belongs to class $\mathcal{K}$ if it is continuous, strictly increasing, and $\alpha(0)=0$. A class $\mathcal{K}$ function belongs to class $\mathcal{K}_\infty$ if $\alpha(x)\rightarrow \infty$ when $x\rightarrow \infty$. We use $\mathbb{P}(\cdot)$ to represent the probability of an event.

\subsection{Gaussian Distribution Temporal Logic}

We consider Gaussian distribution temporal logic (GDTL) \cite{vasile2016control,leahy2019control} whose syntax is defined as follows:
\begin{equation}
    \varphi = True|l\leq 0|\neg\varphi|\varphi_1\land\varphi_2|\varphi_1\mathcal{U}\varphi_2,
\end{equation}
where $l:\mathbb{R}^n\times \mathbb{S}^{n\times n}\rightarrow\mathbb{R}$, $l\leq 0$ is a predicate, and $\mathbb{S}^{n\times n}$ denotes the set of positive semi-definite matrices.

Let $\mathcal{G}_h=\{b:l(b)\leq 0\}$ be the set of belief states such that predicate $l$ is true and $\mathcal{L}_\varphi$ be the set of predicates that appear in a GDTL formula $\varphi$. 

Let $\mathbf{b}=b^0b^1\ldots$ be an infinite sequence of belief states with each $b^i\in\mathbb{R}^n\times \mathbb{S}^{n\times n}$. We denote the suffix $b^tb^{t+1}\ldots$ of $\mathbf{b}$ as $\mathbf{b}^t$. Then a GDTL formula is interpreted as follows:
\begin{itemize}
    \item $\mathbf{b}^t\models True$
    \item  $\mathbf{b}^t\models l\leq 0$ iff $l(b^t)\leq 0$
    \item $\mathbf{b}^t\models\neg\varphi$ iff $\neg(\mathbf{b}^t\models\varphi)$
    \item $\mathbf{b}^t\models\varphi_1\land\varphi_2$ iff $(\mathbf{b}^t\models\varphi_1)\land (\mathbf{b}^t\models\varphi_2)$
    \item $\mathbf{b}^t\models\varphi_1\mathcal{U}\varphi_2$ iff $\exists t'\geq t$ s.t. $(\mathbf{b}^{t'}\models\varphi_2)\land (\mathbf{b}^{t''}\models\varphi_1)$ for all $t''<t'$
\end{itemize}

We introduce the following definition so as to construct an equivalent deterministic Rabin automaton (DRA) representing GDTL formula $\varphi$.
\begin{definition}[\cite{leahy2019control}]\label{def:LTL equiv}
Let $\varphi$ be a GDTL formula. Let $\Tilde{\Pi}$ be an additional finite set of atomic propositions such that $|\mathcal{L}_\varphi|=|\Tilde{\Pi}|$. Let $e:\mathcal{L}_\varphi\rightarrow\Tilde{\Pi}$ be a bijective map. Then GDTL formula $\varphi$ is equivalent to an LTL formula $\Tilde{\varphi}$ defined over atomic proposition set $\Pi\cup\Tilde{\Pi}$, with each predicate $l$ in $\mathcal{L}_\varphi$ being replaced by $e(l)\in\Tilde{\Pi}$.
\end{definition}

Leveraging Definition \ref{def:LTL equiv}, we can represent GDTL formula using an equivalent deterministic Rabin automaton (DRA) defined as follows.
\begin{definition}[Deterministic Rabin Automaton (DRA) \cite{baier2008principles}]\label{def:DRA}
A Deterministic Rabin Automaton (DRA) is a tuple $\mathcal{A}=(Q,\Sigma,\delta,q_0,F)$, where $Q$ is a finite set of states, $\Sigma$ is the finite set of alphabet, $\delta:Q\times\Sigma\mapsto Q$ is a finite set of transitions, $q_0\in Q$ is the initial state, and $F=\{(B(1),\Gamma(1)),\ldots,(B(S),\Gamma(S))\}$ is a finite set of Rabin pairs such that $B(s),\Gamma(s)\subseteq Q$ for all $s=1,\ldots,S$ with $S$ being a positive integer.
\end{definition}

\subsection{Extended Kalman Filter}\label{sec:EKF}

This subsection presents background on extended Kalman filter (EKF) \cite{reif2000stochastic}. Consider a dynamical system
\begin{subequations}\label{eq:prelim dynamics}
\begin{align}
    dx_t &= (f(x_t)+g(x_t)u_t)dt+\sigma_tdW_t,\\
    dy_t &= cx_tdt+\nu_tdV_t
\end{align}
\end{subequations}
where $x_t\in\mathbb{R}^n$ is the system state, and $u_t\in\mathbb{R}^p$ is the control input at time t. Functions $f:\mathbb{R}^n\rightarrow\mathbb{R}^n$ and $g:\mathbb{R}^n\rightarrow\mathbb{R}^{n\times p}$ are locally Lipschitz continuous, $\sigma_t\in\mathbb{R}^{n\times n}$, $W_t$ is an $n$-dimensional Brownian motion, $y_t\in\mathbb{R}^q$ is the output at time $t$, $c\in\mathbb{R}^{q\times n}$, $\nu_t\in\mathbb{R}^{q\times q}$, and $V_t$ is a $q$-dimensional Brownian motion. 

We denote the state estimate at time $t$ as $\hat{x}_t$. Then the dynamics of $\hat{x}_t$ can be represented as
\begin{equation}\label{eq:EKF estimate}
    \hat{x}_t=(f(\hat{x}_t)+g(\hat{x}_t)u_t)dt+K_t(dy_t-c\hat{x}_tdt),
\end{equation}
where $K_t=P_tc^\top R_t^{-1}$ and $R_t=\nu_t\nu_t^\top$. Matrix $P_t$ is the positive definition solution to
\begin{equation}\label{eq:EKF Ricatti}
    \frac{dP}{dt}=A_tP_t+P_tA_t^\top +Q_t-P_tc^\top R_t^{-1}cP_t,
\end{equation}
where $Q_t=\sigma_t\sigma_t^\top$ and $A_t=\frac{\partial \Bar{f}}{\partial x}(\hat{x}_t,u)$ with $\Bar{f}(x,u)=f(x)+g(x)u$.


We make the following assumptions on Eqn. \eqref{eq:prelim dynamics}.
\begin{assumption}\label{assump:SDE conditions}
SDEs in Eqn. \eqref{eq:prelim dynamics} satisfy the following conditions:
\begin{enumerate}
    \item There exist constants $\beta_1$ and $\beta_2$ such that $Q_t\geq \beta_1I$ and $R_t\geq \beta_2I$ for all $t$;
    \item The pair $[\frac{\partial \Bar{f}}{\partial x}(x,u),c]$ is uniformly detectable;
    \item Let $\Delta(x,\hat{x},u)=\Bar{f}(x,u)-\Bar{f}(\hat{x},u)-\frac{\Bar{f}}{\partial x}(x-\hat{x},u)$. Then there exist real numbers $k_\Delta$ and $\epsilon_\Delta$ such that
    \begin{equation*}
        \|\Delta(x,\hat{x},u)\|\leq k_\Delta \|x-\hat{x}\|_2^2
    \end{equation*}
    for all $x$ and $\hat{x}$ satisfying $\|x-\hat{x}\|_2\leq \epsilon_\Delta$.
\end{enumerate}
\end{assumption}
Given Assumption \ref{assump:SDE conditions}, we have the following result.
\begin{lemma}[\cite{reif2000stochastic}]\label{lemma:estimation error}
Suppose the conditions of Assumption \ref{assump:SDE conditions} hold. If there exists $\varepsilon>0$ such that if $Q_t\leq \varepsilon I$ and $R_t\leq \varepsilon I$, then for any $\zeta>0$, there exists $\gamma>0$ such that
\begin{equation}\label{eq:EKF accuracy}
    \mathbb{P}\left(\sup_{t\geq 0}\|x_t-\hat{x}_t\|_2\leq \gamma\right)\geq 1-\zeta.
\end{equation}
\end{lemma}

\subsection{Finite Time Stability in Probability of Stochastic Nonlinear Systems}

In this subsection, we introduce background on finite time stability of stochastic nonlinear systems. Consider a stochastic nonlinear system as follows:
\begin{equation}\label{eq:nonlinear}
    dx_t = f(x_t)dt + g(x_t)dW_t,
\end{equation}
where $x_t\in\mathbb{R}^n$ is the system state, $W_t$ is the $m$-dimensional Brownian motion. Functions $f:\mathbb{R}^n\rightarrow\mathbb{R}^n$ and $g:\mathbb{R}^n\rightarrow\mathbb{R}^{n\times m}$ are measurable continuous function. We then give the definition of finite time stability in probability.
\begin{definition}[Finite Time Stability in Probability \cite{yin2011finite}]
The solution of system \eqref{eq:nonlinear}, denoted as $x(t;x_0)$, is said to be finite time stable in probability if system \eqref{eq:nonlinear} admits a unique solution for any initial state $x_0\in\mathbb{R}^n$ and the following conditions hold:
\begin{enumerate}
    \item \underline{\emph{Finite time attractiveness in probability:}} For every initial state $x_0\neq \mathbf{0}$, the stochastic settling time $\tau_{x_0}=\inf\{t:x(t;x_0)=\mathbf{0}\}$ is finite almost surely, i.e., $\mathbb{P}(\tau_{x_0}<\infty)=1$.
    \item \underline{\emph{Stability in probability:}} For every pair of $\epsilon\in(0,1)$ and $r>0$, there exists some constant $v$ such that 
    \begin{equation}
        \mathbb{P}(|x(t;x_0)|<r,~\forall t\geq 0)\geq 1-\epsilon,
    \end{equation}
    for any $|x_0|<v$.
\end{enumerate}
\end{definition}

Let $V$ be a twice continuously differentiable function. Finite time stability in probability is then certified by the following stochastic Lyapunov theorem.
\begin{theorem}[Stochastic Lyapunov Theorem \cite{yin2011finite}]\label{thm:SCLF}
Assume system \eqref{eq:nonlinear} admits a unique solution. If there exists a twice continuously differentiable function $V:\mathbb{R}^n\rightarrow\mathbb{R}_{\geq 0}$, class $\mathcal{K}_\infty$ functions $\alpha_1$ and $\alpha_2$, positive constants $\gamma>0$ and $\rho\in(0,1)$ such that 
\begin{subequations}
\begin{align}
    &\alpha_1(|x|)\leq V(x)\leq \alpha_2(|x|),\\
    &\frac{\partial V(x)}{\partial x}f(x)+\frac{1}{2}tr\left(g(x)^\top\frac{\partial^2 V(x)}{\partial x^2}g(x)\right) + \gamma\cdot V(x)^\rho\leq 0
\end{align}
\end{subequations}
then the solution of system \eqref{eq:nonlinear} is finite time stable in probability.
\end{theorem}


